Extending Bron Kerbosch for Solving the Maximum Weight Clique Problem

This contribution extends the Bron Kerbosch algorithm for solving the maximum weight clique problem, where continuous-valued weights are assigned to both, vertices and edges. We applied the proposed algorithm to graph matching problems.

==> arxiv1101/config.tex <==

%%% packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{epsf}
\usepackage{makeidx}
%\usepackage{psfrag}
\usepackage{graphicx}
\usepackage{subfigure}
%\usepackage{natbib}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amscd}
%\usepackage{epsfig}



%%% MIT style %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newtheorem{definition}{Definition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{example}{Example}
%\newtheorem{remark}{Remark}
%\newtheorem{notation}{Notation}
%\newtheorem{conjecture}{Conjecture}
%\newcommand{\qed}{\hspace*{\fill} $\blacksquare$}
%\newcommand{\proof}{Proof:\ }


% useful commands
\newcommand{\commentout}[1]{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Local Commands %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% skips and spaces %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\proofskip}{\vspace{3ex}} 
\newcommand{\introskip}{\vspace{3ex}} 
\newcommand{\hstiny}{\hspace{0.5pt}} 



%%% Sets of simple elements %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\B}{\mathbb{B}}                    % binary
\newcommand{\N}{\mathbb{N}}                    % positive integer
\newcommand{\Z}{\mathbb{Z}}                    % integer
\newcommand{\R}{\mathbb{R}}                    % reals
\newcommand{\C}{\mathbb{C}}                    % complex
\newcommand{\E}{\mathbb{E}}                    % Euclidean vector space   
% if superscript is required:
%^{\raisebox{1pt}{${\scriptstyle u}$}}}

%%% Functions and Operators %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Brackets
\newcommand{\abs}[1]{\mathop{\left\lvert #1 \right\rvert}} 
\newcommand{\args}[1]{\mathop{\left( #1 \right)}} 
\newcommand{\inner}[1]{\mathop{\left\langle #1 \right\rangle}}
\newcommand{\norm}[1]{\mathop{\left\lVert #1 \right\rVert}}
\newcommand{\cbrace}[1]{\mathop{\left\{ #1 \right\}}}
\newcommand{\bracket}[1]{\mathop{\left[ #1 \right]}}

\newcommand{\absS}[2]{\mathop{\left\lvert #1 \right\rvert#2}} 
\newcommand{\argsS}[2]{\mathop{\left( #1 \right)#2}} 
\newcommand{\innerS}[2]{\mathop{\left\langle #1 \right\rangle#2}}
\newcommand{\normS}[2]{\mathop{\left\lVert #1 \right\rVert#2}}
\newcommand{\cbraceS}[2]{\mathop{\left\{ #1 \right\}#2}}
\newcommand{\bracketS}[2]{\mathop{\left[ #1 \right]#2}}
 
% Operators
\DeclareMathOperator{\aff}{aff}                % affine hull
\DeclareMathOperator{\bd}{bd}                  % boundary
\DeclareMathOperator{\cl}{cl}                  % closure
\DeclareMathOperator{\conv}{con}               % convex hull
\DeclareMathOperator{\cone}{cone}              % conic hull

\DeclareMathOperator{\Aut}{Aut}                % automorphism group
\DeclareMathOperator{\id}{id}                  % identity function
\DeclareMathOperator{\interior}{int}           % interior
\DeclareMathOperator{\Irr}{Irr}                % set of irregular structures
\DeclareMathOperator{\diag}{diag}              % diagonal
\DeclareMathOperator{\dom}{dom}                % domain
\DeclareMathOperator{\relative}{rel}           % relative
\DeclareMathOperator{\Span}{Span}              % vector space span
\DeclareMathOperator{\supp}{supp}              % support of a vector
\DeclareMathOperator{\tr}{tr}                  % trace
\newcommand{\T}{\mathop{\mathsf{T}}}           % transpose 
\DeclareMathOperator{\VEC}{vec}                % vector operator of matrices
\DeclareMathOperator{\MAT}{mat}                % matrix operator of vectors

\DeclareMathOperator{\wdeg}{wdeg}       

% transfer functions
\DeclareMathOperator{\LT}{LT}                  % linear threshold function
\DeclareMathOperator{\sgn}{sgn}                % signum function


%%% Fonts %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\abb}[1]{#1}                       % abbreviations
\newcommand{\A}[1]{$\mbox{\tt #1}$}            % algorithms
\renewcommand{\S}[1]{{\mathcal{#1}}}           % arbitrary sets
                                               % vector
\def\vec#1{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
{\mbox{\boldmath$\textstyle#1$}}
{\mbox{\boldmath$\scriptstyle#1$}}
{\mbox{\boldmath$\scriptscriptstyle#1$}}}

%%% Abbreviations %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\eps}{\varepsilon}                 % varepsilon
                                               % index fraction for sums etc
\newcommand{\indexfrac}[2]{\genfrac{}{}{0pt}{2}{#1}{#2}}

%%% Mathematical accents %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\widebar}[1]{\overline{\!#1}}   % wide bar 



%%% Environment Algorithm %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\atab}[1]{\hspace*{#1em}}
\newcommand{\aseptab}{\hspace*{0.5em}--\hspace{0.5em}}
\newcounter{algorithm_counter}
\setcounter{algorithm_counter}{0}
\newenvironment{algorithm}[1]{
\refstepcounter{algorithm_counter}
\setlength{\parindent}{0\parindent}
\vspace{2ex}
\begin{minipage}{\textwidth}
\rule{\textwidth}{5\arrayrulewidth}\\
\begin{footnotesize}
{\bf Algorithm \arabic{algorithm_counter}} (#1) \\
\rule[+1.5ex]{\textwidth}{\arrayrulewidth}

\vspace{-1.5ex}

}%
{
\\[-1.5ex]
\rule{\textwidth}{\arrayrulewidth}
%\end{sf}
\end{footnotesize}
\end{minipage}
\setlength{\parindent}{\parindent}
}


\newenvironment{algorithmwindow}{
\setlength{\parindent}{0\parindent}
\vspace{2ex}
\begin{minipage}{0.45\textwidth}
\begin{footnotesize}
%\begin{sf}
\rule[+1.5ex]{\textwidth}{\arrayrulewidth}

\vspace{-1.5ex}

}%
{
\\[-1.5ex]
\rule{\textwidth}{\arrayrulewidth}
%\end{sf}
\end{footnotesize}
\end{minipage}
\setlength{\parindent}{\parindent}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



